V2X-Radar: A Multi-modal Dataset with 4D Radar for Cooperative Perception

Modern autonomous vehicle perception systems often struggle with occlusions and limited perception range. Previous studies have demonstrated the effectiveness of cooperative perception in extending the perception range and overcoming occlusions, thereby enhancing the safety of autonomous driving. In recent years, a series of cooperative perception datasets have emerged; however, these datasets primarily focus on cameras and LiDAR, neglecting 4D Radar, a sensor used in single-vehicle autonomous driving to provide robust perception in adverse weather conditions. In this paper, to bridge the gap created by the absence of 4D Radar datasets in cooperative perception, we present V2X-Radar, the first large-scale, real-world multi-modal dataset featuring 4D Radar. V2X-Radar dataset is collected using a connected vehicle platform and an intelligent roadside unit equipped with 4D Radar, LiDAR, and multi-view cameras. The collected data encompasses sunny and rainy weather conditions, spanning daytime, dusk, and nighttime, as well as various typical challenging scenarios. The dataset consists of 20K LiDAR frames, 40K camera images, and 20K 4D Radar data, including 350K annotated boxes across five categories. To support various research domains, we have established V2X-Radar-C for cooperative perception, V2X-Radar-I for roadside perception, and V2X-Radar-V for single-vehicle perception. Furthermore, we provide comprehensive benchmarks across these three sub-datasets. We will release all datasets and benchmark codebase at https://huggingface.co/datasets/yanglei18/V2X-Radar and https://github.com/yanglei18/V2X-Radar.

==> latex/fig/annotation_density.tex <==
\begin{figure}[h!t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/annotation_density.pdf}
	\caption{
	\textbf{Number of annotations per collaborative sample.} 
	}
\label{fig:annotation_density}
\end{figure}

==> latex/fig/rebuttal_distribution.tex <==
\begin{figure}[h!t]
\centering
\vspace{-0.3cm}
\includegraphics[width=0.47\textwidth]{figures/rebuttal_distribution.pdf}
% \caption{\textbf{Data analysis of our V2X-Radar dataset.}}
\label{fig:rebuttal_distribution}
\vspace{-0.8cm}
\end{figure}

==> latex/fig/teaser.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
\centering
\captionsetup{type=figure}
\vspace{-0.38cm}
\begin{center}
\includegraphics[width=0.99\textwidth]{figures/teaser-v2.pdf}
\end{center}
\setlength{\belowcaptionskip}{-0.005cm} 
\captionof{figure}{
\textbf{A data frame sampled from the V2X-Radar dataset}. Each sample includes data from three sensors: (1) dense point clouds (\textcolor[RGB]{120,120,120}{gray} points) from roadside and vehicle-side LiDAR; (2) sparse point clouds (\textcolor[RGB]{102,255,170}{green} and \textcolor[RGB]{24,116,255}{blue} points) with Doppler information from the roadside and vehicle-mounted 4D Radar; (3) RGB images (top row) from the vehicle’s camera and multi-view roadside cameras. All sensors are temporally and spatially synchronized. Each data frame is manually annotated with 3D boxes across five categories. % each category being represented by a unique color.
}
\label{fig:teaser}
%\vspace{0.15cm}
\end{center}
}]



==> latex/tab/sensor_specifications_v2.tex <==
\begin{table*}[h!t]
\small
\centering
 \caption{Key Sensor Specifications in V2X-Real Dataset. Infra means infrastructure.}
\begin{tabular}{l|l|l|p{9.3cm}}
\toprule
\textbf{Agent}&\textbf{Sensor}&\textbf{Sensor Model} & \textbf{Details}  \\
\toprule
\multirow{8}{*}{Infra}&LiDAR& RoboSense  RS-Ruby-80 ($\times$1) & 80 beams, 10Hz capture frequency, $360^\circ$ horizontal FOV, $-25^\circ \text{to} +25^\circ$vertical FOV, $\leq$ 200m range;\\
&Camera & Basler acA1920-40gc ($\times$3) &RGB, 10Hz capture frequency, 1536×864 resolution; \\ 
&4D Radar& OCULI EAGLE ($\times$1) & $ 79.0$ GHz, $0.86$m range precision, $-56.5^\circ \text{to} +56.5^\circ$ horizontal FOV, $-22.5^\circ \text{to} +22.5^\circ$ vertical FOV,  $\leq 400$m range;\\
&C-V2X Unit & VU4004 ($\times$1) & PC5/4G LTE/V2X Protocol; \\ 
&GPS/IMU & XW-GI5651 ($\times$1) & 1000Hz update rate, Double-Precision; \\ 
\midrule
      \multirow{8}{*}{Vehicle}&LiDAR& RoboSense  RS-Ruby-80 ($\times$1) & 80 beams, 10Hz capture frequency, $360^\circ$ horizontal FOV, $-25^\circ \text{to} +25^\circ$ vertical FOV,$\leq$ 200mrange;\\
&Camera & Basler acA1920-40gc ($\times$1) &RGB, 10Hz capture frequency, 1920×1080 resolution; \\ 
&4D Radar& Arbe Phoenix ($\times$1) & 77GHz, 0.6m range precision, $-50^\circ \text{to} +50^\circ$ horizontal FOV, $-15^\circ \text{to} +15^\circ$ vertical FOV, $\leq$ 300m range
;\\
&C-V2X Unit & VU4004 ($\times$1) & PC5/4G LTE/V2X Protocol; \\ 
&GPS/IMU & XW-GI5651 ($\times$1) & 1000Hz update rate, Double-Precision; \\ 
     \bottomrule
\end{tabular}
\label{tab:sensor_specifications}  
\end{table*}


